TensorQC: Towards Scalable Distributed Quantum Computing via Tensor Networks

A quantum processing unit (QPU) must contain a large number of high quality qubits to produce accurate results for problems at useful scales. In contrast, most scientific and industry classical computation workloads happen in parallel on distributed systems, which rely on copying data across multiple cores. Unfortunately, copying quantum data is theoretically prohibited due to the quantum non-cloning theory. Instead, quantum circuit cutting techniques cut a large quantum circuit into multiple smaller subcircuits, distribute the subcircuits on parallel QPUs and reconstruct the results with classical computing. Such techniques make distributed hybrid quantum computing (DHQC) a possibility but also introduce an exponential classical co-processing cost in the number of cuts and easily become intractable. This paper presents TensorQC, which leverages classical tensor networks to bring an exponential runtime advantage over state-of-the-art parallelization post-processing techniques. As a result, this paper demonstrates running benchmarks that are otherwise intractable for a standalone QPU and prior circuit cutting techniques. Specifically, this paper runs six realistic benchmarks using QPUs available nowadays and a single GPU, and reduces the QPU size and quality requirements by more than $10\times$ over purely quantum platforms.

==> text/results/fidelity.tex <==
\subsection{Fidelity on Real Device}
\begin{figure}[t]
    \centering
    \includegraphics[width=.85\linewidth]{figures/fidelity.pdf}
    \caption{Fidelity comparison of cut versus uncut on the $27$-qubit $IBM\_Montreal$ QPU.
    Figure shows the error obtained via cutting as a percentage of that of uncut.
    Each data point is the average of $3$ trials.
    $Regular$ benchmark experiences error reduction of nearly $60\%$.
    $GHZ$ has $15\%$ and $W\_state$ has $30\%$ reductions.}
    \label{fig:fidelity}
\end{figure}

TensorQC generally produces more accurate results than without cutting.
Figure~\ref{fig:fidelity} cuts and runs several benchmarks at various sizes on the $27$-qubit IBM Montreal QPU.
TensorQC uses at most $10$-qubit subcircuits.
The same set of benchmarks also run as is without cutting on the same IBM QPU.
Classical simulation then produces the ground truth to verify both types of outputs.

The accuracy comparison is quantified by the relative error of TensorQC as a percentage of that of uncut.
Specifically, we compute
\begin{equation*}
    \frac{e(\textrm{TensorQC},\textrm{Ground Truth})}{e(\textrm{Uncut},\textrm{Ground Truth})}
\end{equation*}
where $e$ is the MSE defined in Equation~\ref{eq:mse}.

Figure~\ref{fig:fidelity} shows that the accuracy of the various benchmarks improved under cutting.
This is likely due to the fact that TensorQC replaces the noisy quantum links with noiseless classical post-processing at key locations.
In addition, QPUs produce more accurate results for the small subcircuits than the large uncut circuits.
This is due to a myriad of software and hardware factors including compiler performance, crosstalk and decoherence.
Since QPU noise is the only source of error in TensorQC,
smaller QPU burden is generally favored to produce more accurate overall results.

==> text/results/highlight.tex <==
\subsection{Making the Impossible Possible}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/cut_visual.pdf}
    \caption{Subcircuit partitions to run a $196$-qubit quantum supremacy circuit.
    DAG shows the $2$-qubit quantum gates, with colors indicating the subcircuits they belong in.
    TensorQC runs the otherwise intractable circuit with up to $15$-qubit QPUs and a single GPU.
    Figure~\ref{fig:total_runtime_estimation} estimates that the total runtime to execute $1$ million arbitrary quantum states is $50$ hours.}
    \label{fig:supremacy_highlight}
\end{figure}

Figure~\ref{fig:supremacy_highlight} shows the subcircuit partition results of the $196$-qubit $Supremacy$ circuit.
Without cutting, the benchmark requires a $196$-qubit QPU that is capable of reliably running $1.3k$ gates.
TensorQC instead cuts the benchmark into $52$ subcircuits of at most $15$ qubits and $60$ gates.
Figure~\ref{fig:total_runtime_estimation} estimates that the total runtime to execute the benchmark is $50$ hours.
Section~\ref{sec:runtime_results} explains that this estimation based on Equation~\ref{eq:cut_objective} tends to overestimate.
However, the estimation predicts a rough sense of timescale to run the otherwise intractable benchmark.
This is the largest demonstration of the $Supremacy$ benchmark to the best of our knowledge.
